Adwords in a Panorama

Three decades ago, Karp, Vazirani, and Vazirani (STOC 1990) defined the online matching problem and gave an optimal $1-\frac{1}{e} \approx 0.632$-competitive algorithm. Fifteen years later, Mehta, Saberi, Vazirani, and Vazirani (FOCS 2005) introduced the first generalization called AdWords driven by online advertising and obtained the optimal $1-\frac{1}{e}$ competitive ratio in the special case of small bids. It has been open ever since whether there is an algorithm for general bids better than the $0.5$-competitive greedy algorithm. This paper presents a $0.5016$-competitive algorithm for AdWords, answering this open question on the positive end. The algorithm builds on several ingredients, including a combination of the online primal dual framework and the configuration linear program of matching problems recently explored by Huang and Zhang (STOC 2020), a novel formulation of AdWords which we call the panorama view, and a generalization of the online correlated selection by Fahrbach, Huang, Tao, and Zadimorghaddam (FOCS 2020) which we call the panoramic online correlated selection.

==> hybrid-lp.tex <==
\subsection{Optimization of The Ratio via LP}
\label{subsec:hybrid-lp}
\begin{itemize}
    \item $\Tilde{k_a}(y) = k^{\min} + 1$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^B$, $h(y) \in Y^B$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min} + 1} \Delta\alpha_L^R(j) + 1 - x(k^{\min}) - \Delta\alpha_L^D(k^{\min}+1)\\
    &+ \sum_{j=1}^{k^{\min}} \Delta\alpha_R^R(j) + 1 - x(k^{\min} - 1) - \Delta\alpha_R^D(k^{\min})
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min}$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^B$, $h(y) \in Y^B$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}} \Delta\alpha_L^R(j) + 1 - x(k^{\min}) - \Delta\alpha_L^D(k^{\min})\\
    &+ \sum_{j=1}^{k^{\min}} \Delta\alpha_R^R(j) + 1 - x(k^{\min} - 1) - \Delta\alpha_R^D(k^{\min})
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min} + 1$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^B$, $h(y) \in Y^F$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}+1} \Delta\alpha_L^R(j) + 1 - x(k^{\min}) - \Delta\alpha_L^D(k^{\min}+1)\\
    &+ \sum_{j=1}^{k^{\min}-1} \Delta\alpha_R^R(j) + \Delta\alpha_R^D(k^{\min})
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min}$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^B$, $h(y) \in Y^F$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}} \Delta\alpha_L^R(j) + 1 - x(k^{\min}-1) - \Delta\alpha_L^D(k^{\min})\\
    &+ \sum_{j=1}^{k^{\min}-1} \Delta\alpha_R^R(j) + \Delta\alpha_R^D(k^{\min})
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min} + 1$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^B$, $h(y) \in Y^N$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min} + 1} \Delta\alpha_L^R(j) + 1 - x(k^{\min}) - \Delta\alpha_L^D(k^{\min} + 1)\\
    &+ \sum_{j=1}^{k^{\min}-1} \Delta\alpha_R^R(j) + \frac{1 - x(k^{\min}-1)}{2} - \Delta\alpha_R^R(k^{\min})
    \end{align*}
    
    % \item $\Tilde{k_a}(y) = k^{\min}$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^B$, $h(y) \in Y^N$.
    % \begin{align*}
    % g(y) + g(h(y)) =
    % & \sum_{j=1}^{k^{\min}} \Delta\alpha_L^R(j) + 1 - x(k^{\min}-1) - \Delta\alpha_L^D(k^{\min})\\
    % &+ \sum_{j=1}^{k^{\min}-1} \Delta\alpha_R^R(j) + \frac{1 - x(k^{\min}-1)}{2} - \Delta\alpha_R^R(k^{\min})
    % \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min} + 1$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^F$, $h(y) \in Y^B$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}} \Delta\alpha_L^R(j) + \Delta\alpha_L^D(k^{\min}+1)\\
    &+ \sum_{j=1}^{k^{\min}} \Delta\alpha_R^R(j) + 1 - x(k^{\min}-1) - \Delta\alpha_R^D(k^{\min})
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min}$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^F$, $h(y) \in Y^B$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}-1} \Delta\alpha_L^R(j) + \Delta\alpha_L^D(k^{\min})\\
    &+ \sum_{j=1}^{k^{\min}} \Delta\alpha_R^R(j) + 1 - x(k^{\min}-1) - \Delta\alpha_R^D(k^{\min})
    \end{align*}
    
    % \item $\Tilde{k_a}(y) = k^{\min} + 1$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^F$, $h(y) \in Y^N$.
    % \begin{align*}
    % g(y) + g(h(y)) =
    % & \sum_{j=1}^{k^{\min}} \Delta\alpha_L^R(j) + \Delta\alpha_L^D(k^{\min}+1)\\
    % &+ \sum_{j=1}^{k^{\min}} \Delta\alpha_R^R(j) + \frac{1 - x(k^{\min})}{2} - \Delta\alpha_R^R(k^{\min} + 1)
    % \end{align*}
% \end{itemize}
% \end{multicols}
% \begin{multicols}{2}
% \begin{itemize}
    \item $\Tilde{k_a}(y) = k^{\min}$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^F$, $h(y) \in Y^N$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}-1} \Delta\alpha_L^R(j) + \Delta\alpha_L^D(k^{\min})\\
    &+ \sum_{j=1}^{k^{\min}} \Delta\alpha_R^R(j) + \frac{1 - x(k^{\min})}{2} - \Delta\alpha_R^R(k^{\min} + 1)
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min} + 1$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^N$, $h(y) \in Y^F$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}+1} \Delta\alpha_L^R(j) + \frac{1 - x(k^{\min+1})}{2} - \Delta\alpha_L^R(k^{\min}+2)\\
    &+ \sum_{j=1}^{k^{\min}-1} \Delta\alpha_R^R(j) + \Delta\alpha_R^D(k^{\min})
    \end{align*}
    
    % \item $\Tilde{k_a}(y) = k^{\min}$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^N$, $h(y) \in Y^F$.
    % \begin{align*}
    % g(y) + g(h(y)) =
    % & \sum_{j=1}^{k^{\min}} \Delta\alpha_L^R(j) + \frac{1 - x(k^{\min})}{2} - \Delta\alpha_L^R(k^{\min}+1)\\
    % &+ \sum_{j=1}^{k^{\min}-1} \Delta\alpha_R^R(j) + \Delta\alpha_R^D(k^{\min})
    % \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min} + 1$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^N$, $h(y) \in Y^B$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}+1} \Delta\alpha_L^R(j) + \frac{1 - x(k^{\min})}{2} - \Delta\alpha_L^R(k^{\min}+1)\\
    &+ \sum_{j=1}^{k^{\min}-1} \Delta\alpha_R^R(j) + \Delta\alpha_R^D(k^{\min})
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min}$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^N$, $h(y) \in Y^B$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}} \Delta\alpha_L^R(j) + \frac{1 - x(k^{\min}-1)}{2} - \Delta\alpha_L^R(k^{\min})\\
    &+ \sum_{j=1}^{k^{\min}-1} \Delta\alpha_R^R(j) + \Delta\alpha_R^D(k^{\min})
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min} + 1$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^N$, $h(y) \in Y^N$, $N = \{i\}$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}+1} \Delta\alpha_L^R(j) + \Delta x(k^{\min}+2) - \Delta\alpha_L^R(k^{\min}+2)\\
    &+ \sum_{j=1}^{k^{\min}} \Delta\alpha_R^R(j) + \Delta x(k^{\min}+1) - \Delta\alpha_L^R(k^{\min}+1)
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min}$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^N$, $h(y) \in Y^N$, $N = \{i\}$.
    \begin{align*}
    g(y) + g(h(y)) =
    & \sum_{j=1}^{k^{\min}+1} \Delta\alpha_L^R(j) + \Delta x(k^{\min}+1) - \Delta\alpha_L^R(k^{\min}+1)\\
    &+ \sum_{j=1}^{k^{\min}} \Delta\alpha_R^R(j) + \Delta x(k^{\min}+1) - \Delta\alpha_R^R(k^{\min}+1)
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min} + 1$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^N$, $h(y) \in Y^N$, $N = \{i_1,i_2\}$
    \begin{align*}
    g(y) + g(h(y)) \geq
    &\sum_{j=1}^{k^{\min}+1} \Delta\alpha_L^R(j) + \frac{1 - x(k^{\min})}{2} - \Delta\alpha_R^R(k^{\min}+1)\\
    &+ sum_{j=1}^{k^{\min}} \Delta\alpha_L^R(j) + \frac{1 - x(k^{\min})}{2} - \Delta\alpha_R^R(k^{\min}+1)
    \end{align*}
    
    \item $\Tilde{k_a}(y) = k^{\min}$,  $\Tilde{k_a}(h(y)) = k^{\min}$, $y\in Y^N$, $h(y) \in Y^N$.$N = \{i_1,i_2\}$
    \begin{align*}
    g(y) + g(h(y)) \geq
    & \sum_{j=1}^{k^{\min}} \Delta\alpha_L^R(j) + \frac{1 - x(k^{\min})}{2} - \Delta\alpha_L^R(k^{\min}+1)\\
    &+ \sum_{j=1}^{k^{\min}} \Delta\alpha_R^R(j) + \frac{1 - x(k^{\min})}{2} - \Delta\alpha_L^R(k^{\min}+1)
    \end{align*}
    
\end{itemize}
% \end{multicols}

